Freezer: A Specialized NVM Backup Controller for Intermittently-Powered Systems

The explosion of IoT and wearable devices determined a rising attention towards energy harvesting as source for powering these systems. In this context, many applications cannot afford the presence of a battery because of size, weight and cost issues. Therefore, due to the intermittent nature of ambient energy sources, these systems must be able to save and restore their state, in order to guarantee progress across power interruptions. In this work, we propose a specialized backup/restore controller that dynamically tracks the memory accesses during the execution of the program. The controller then commits the changes to a snapshot in a Non-Volatile Memory (NVM) when a power failure is detected. Our approach does not require complex hybrid memories and can be implemented with standard components. % and integrated in any MCU with Results on a set of benchmarks show an average $8\times$ reduction in backup size. Thanks to our dedicated controller, the backup time is further reduced by more than $100\times$, with an area and power overhead of only 0.4\% and 0.8\%, respectively, w.r.t. a low-end IoT node.

==> Freezer-TCAD Revised Version/bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{davide}}]{Davide Pala}
%\begin{IEEEbiography}{Davide Pala}
received the B.Sc. and M.Sc. degrees in Computer Engineering from Politecnico di Torino, Torino, Italy, in 2015 and 2017, respectively.
He is currently pursuing the Ph.D. degree in computer science with the University of Rennes, Rennes, France, under the supervision of O. Sentieys and I. Miro-Panades.
His current research interests include embedded systems architectures, non-volatile processor, non-volatile memory, energy harvesting systems and intermittent computing. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ivan}}]{Ivan Miro-Panades}
(M’17) received a M.Sc. in telecommunication engineering from the Technical University of Catalonia (Barcelona, Spain) in 2002, a M.Sc. and a PhD in computer science from the Univ. Pierre \& Marie Curie (Paris, France) in 2004 and 2008, respectively. 
Dr. Miro-Panades worked at Philips Research and ST Microelectronics before joining in 2008 CEA, Grenoble, France, where he is currently a Research Engineer in digital integrated circuits. His main research interests are AI, IoT, energy-efficient systems, and Fmax/Vmin tracking. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{olivier}}]{Olivier Sentieys} (M’94) is Professor at the University of Rennes, France, holding an INRIA Research Chair on Energy-Efficient Computing Systems. 
%He is leading the Cairn team. 
%From 2012 to 2017 he was on secondment at INRIA as a Senior Research Director. 
He received the M.Sc. and Ph.D degrees in Electrical Engineering (signal processing) from the University of Rennes in 1990 and 1993 respectively.
%His research interests are in the area of computer architectures, embedded systems and signal processing, with a focus on system-level design, energy-efficiency, reconfigurable systems, hardware acceleration, approximate computing, and power management of energy harvesting sensor networks. 
His research interests are in the area of computer architectures and embedded systems, with a focus on system-level design, hardware acceleration, approximate computing, energy harvesting sensor networks. 
%He authored or co-authored more than 250 journal or conference papers, holds 6 patents, and served in the technical committees of several international IEEE/ACM/IFIP conferences.
\end{IEEEbiography}



% if you will not have a photo at all:
%\begin{IEEEbiographynophoto}{John Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

%\begin{IEEEbiographynophoto}{Jane Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

==> bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{davide}}]{Davide Pala}
%\begin{IEEEbiography}{Davide Pala}
received the B.Sc. and M.Sc. degrees in Computer Engineering from Politecnico di Torino, Torino, Italy, in 2015 and 2017, respectively.
He is currently pursuing the Ph.D. degree in computer science with the University of Rennes, Rennes, France, under the supervision of O. Sentieys and I. Miro-Panades.
His current research interests include embedded systems architectures, non-volatile processor, non-volatile memory, energy harvesting systems and intermittent computing. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ivan}}]{Ivan Miro-Panades}
(M’17) received a M.Sc. in telecommunication engineering from the Technical University of Catalonia (Barcelona, Spain) in 2002, a M.Sc. and a PhD in computer science from the Univ. Pierre \& Marie Curie (Paris, France) in 2004 and 2008, respectively. 
Dr. Miro-Panades worked at Philips Research and ST Microelectronics before joining in 2008 CEA, Grenoble, France, where he is currently a Research Engineer in digital integrated circuits. His main research interests are AI, IoT, energy-efficient systems, and Fmax/Vmin tracking. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{olivier}}]{Olivier Sentieys} (M’94) is Professor at the University of Rennes, France, holding an INRIA Research Chair on Energy-Efficient Computing Systems. 
%He is leading the Cairn team. 
%From 2012 to 2017 he was on secondment at INRIA as a Senior Research Director. 
He received the M.Sc. and Ph.D degrees in Electrical Engineering (signal processing) from the University of Rennes in 1990 and 1993 respectively.
%His research interests are in the area of computer architectures, embedded systems and signal processing, with a focus on system-level design, energy-efficiency, reconfigurable systems, hardware acceleration, approximate computing, and power management of energy harvesting sensor networks. 
His research interests are in the area of computer architectures and embedded systems, with a focus on system-level design, hardware acceleration, approximate computing, energy harvesting sensor networks. 
%He authored or co-authored more than 250 journal or conference papers, holds 6 patents, and served in the technical committees of several international IEEE/ACM/IFIP conferences.
\end{IEEEbiography}



% if you will not have a photo at all:
%\begin{IEEEbiographynophoto}{John Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

%\begin{IEEEbiographynophoto}{Jane Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
